Trade-offs in Large-Scale Distributed Tuplewise Estimation and Learning

The development of cluster computing frameworks has allowed practitioners to scale out various statistical estimation and machine learning algorithms with minimal programming effort. This is especially true for machine learning problems whose objective function is nicely separable across individual data points, such as classification and regression. In contrast, statistical learning tasks involving pairs (or more generally tuples) of data points - such as metric learning, clustering or ranking do not lend themselves as easily to data-parallelism and in-memory computing. In this paper, we investigate how to balance between statistical performance and computational efficiency in such distributed tuplewise statistical problems. We first propose a simple strategy based on occasionally repartitioning data across workers between parallel computation stages, where the number of repartitioning steps rules the trade-off between accuracy and runtime. We then present some theoretical results highlighting the benefits brought by the proposed method in terms of variance reduction, and extend our results to design distributed stochastic gradient descent algorithms for tuplewise empirical risk minimization. Our results are supported by numerical experiments in pairwise statistical estimation and learning on synthetic and real-world datasets.

==> subfiles/metainfo.tex <==
% !TEX root = ../main-pairs-ECML.tex

%
\title{Trade-offs in Large-Scale Distributed Tuplewise Estimation and
Learning}
%
%\titlerunning{Abbreviated paper title}
% If the paper title is too long for the running head, you can set an abbreviated paper title here 
\author{Robin Vogel\inst{1,2} \and Aur\'elien Bellet\inst{3} \and Stephan
Cl\'emen\c{c}on\inst{1} \and
Ons Jelassi\inst{1} \and Guillaume Papa\inst{1}}
%
\authorrunning{R. Vogel et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{Telecom ParisTech, LTCI, Universit\'e Paris Saclay, France\\
\email{first.last@telecom-paristech.fr}\and IDEMIA, France\\
\email{first.last@idemia.fr}\and INRIA, France\\
\email{first.last@inria.fr} 
}
%\institute{IDEMIA, France\\
%\email{robin.vogel@idemia.com}}
\maketitle              % typeset the header of the contribution
%
\begin{abstract}
The development of cluster computing frameworks has
allowed practitioners to scale out various statistical estimation and machine
learning algorithms with minimal programming effort. This is especially true for machine learning problems whose objective function is nicely separable across individual data points, such as classification and regression.
In contrast, statistical learning tasks involving pairs (or
more generally tuples) of data points --- such as metric learning,
clustering or ranking --- do not lend themselves as easily to
data-parallelism
and in-memory computing.
% Indeed, naive implementations for these problems lead to solutions that are
% either scalable but poorly accurate, or accurate but prohibitively expensive due communication costs and/or disk spills.
In this paper, we investigate how to balance between statistical performance
and computational efficiency in such distributed tuplewise statistical
problems. We first propose a simple strategy based on occasionally
repartitioning
data across workers between parallel computation stages, where the number of
repartitioning steps rules the trade-off between accuracy and runtime. We then
present some theoretical results highlighting the benefits brought by the
proposed method in terms of variance reduction, and extend our results to
design
distributed stochastic gradient descent algorithms for tuplewise
empirical
risk minimization.
Our results are supported by numerical experiments in pairwise
statistical estimation and learning on synthetic and real-world datasets.

% Whereas the recent development of cluster computing frameworks such as Apache Spark has permitted to scale-up significantly various machine-learning algorithms, for classification/regression in particular, many statistical learning tasks, including popular approaches for metric learning, clustering or ranking, involve considering pairs (or tuples, more generally) of data points and do not lend themselves the implicit data splitting enabling parallelism and avoiding in-memory limitations. It is indeed far from straightforward to develop efficient parallel and distributed approaches for pairwise learning: a naive implementation of dedicated statistical methods restricted to a large collection of small data subsets combined with an aggregation procedure may guarantee scalability though seriously damage statistical accuracy (the statistical population of pairs within each local batch being then too small regarding the objectives of the estimation/prediction task), while sampling strategies mimicking centralized methods and guaranteeing the representativeness of the ensemble of pairs over which the algorithm passes might spill to disk, by writing and reading temporary data (\textit{i.e.} indices of the training data picked by the sampling algorithm) too frequently. It is the goal of this paper to investigate how to balance between statistical performance and computational efficiency in large-scale pairwise statistical problems using Apache Spark. We develop a framework proving that an optimal tradeoff
% can be achieved by shuffling the data between parallel-computation phases, so as to re-distribute them into a new partition, at a certain frequency. The preliminary theoretical results, related to the dramatic improvement  an appropriate data shuffling stage can lead to, we established are also supported by strong empirical evidence, as illustrated by the numerical experiments displayed in this paper.

\keywords{Distributed Machine Learning \and Distributed Data
Processing \and $U$-Statistics \and Stochastic Gradient Descent \and AUC
Optimization}
\end{abstract}

